Leveraging Large Language Models for NLG Evaluation: Advances and Challenges

In the rapidly evolving domain of Natural Language Generation (NLG) evaluation, introducing Large Language Models (LLMs) has opened new avenues for assessing generated content quality, e.g., coherence, creativity, and context relevance. This paper aims to provide a thorough overview of leveraging LLMs for NLG evaluation, a burgeoning area that lacks a systematic analysis. We propose a coherent taxonomy for organizing existing LLM-based evaluation metrics, offering a structured framework to understand and compare these methods. Our detailed exploration includes critically assessing various LLM-based methodologies, as well as comparing their strengths and limitations in evaluating NLG outputs. By discussing unresolved challenges, including bias, robustness, domain-specificity, and unified evaluation, this paper seeks to offer insights to researchers and advocate for fairer and more advanced NLG evaluation techniques.

==> 0-new_papers.tex <==
Don’t Rank, Combine! Combining Machine Translation Hypotheses Using Quality Estimation

==> table_tune.tex <==
\begin{table*}[t!]
    \centering
    \small
    \resizebox{\textwidth}{!}{
    \begin{tabular}{cp{0.25cm}p{0.25cm}p{0.25cm}p{0.25cm}p{0.25cm}p{0.25cm}p{0.25cm}p{0.3cm}cp{1.4cm}c}
        \toprule
         Metric & MT & AS & DG & IC & D2T & SG & GE & REF & LLMs	& Protocol	& data\\
         \midrule

         \midrule
         \multicolumn{12}{c}{ \emph{Tuning-based Evaluation} }\\
         \midrule

        PRISM~\cite{thompson-post-2020-automatic} & \checkmark & * & * & * & * & * & * & \checkmark & Transformer & Prob & NONE \\

        T5Score~\cite{qin2022t5score} & \checkmark & \checkmark & * & * & * & *& & \checkmark & T5 & Prob & NONE \\
        TrueTeacher~\cite{gekhman2023trueteacher} & * & \checkmark & * & & * & * & * & & T5 & Likert & CON\\
        \cdashlinelr{1-12}
        
         Attscore~\cite{yue2023automatic} & & & & & & & \checkmark & & 
          \begin{tabular}[c]{@{}l@{}}  Roberta/T5/GPT2 \\ LLaMA/Vicuna \end{tabular} 
         & Likert & fine-grain errors [F1] \\
         \cdashlinelr{1-12}
        
         
         AUTO-J~\cite{li2023generative} & * & * & * & & * & * & * & & LLaMA & Likert/Pairwise & 
            critique-then-score
         \\
         \cdashlinelr{1-12}

         PERSE~\cite{wang2023learning} & & * & * & * & & \checkmark & * & \checkmark & LLaMA & Likert/Pairwise & give example- explanation  \\
         
         PandaLM~\cite{wang2023pandalm} & * & * & * & & * & * & \checkmark & & LLaMA & Pairwise & reason+results\\
         %ECT~\cite{} \\
         TIGERScore~\cite{jiang2023tigerscore} & \checkmark & \checkmark & * & & \checkmark & \checkmark & \checkmark & & LLaMA & Advanced & error type — score  \\
         INSTRUCTSCORE~\cite{xu2023instructscore} & \checkmark & * & * & * & * & * & * & \checkmark & LLaMA & Advanced & error type — score \\
         Prometheus~\cite{kim2023prometheus} & * & * & * &  & * & * & \checkmark & & LLaMA-2 & Likert/Pairwise & feedback(explanation)/score \\
         CritiqueLLM~\cite{ke2023critiquellm} & * & * & * &  & * & * & \checkmark & & ChatGLM & Likert & multiturn--explanation/score \\
         \bottomrule
    \end{tabular}
    }
    \caption{Automatic metrics proposed (\checkmark) and adopted (*) for various NLG tasks. 
    }
    \label{tab:tune}
\end{table*}

